AutoGen: Enabling Next-Gen LLM Applications via Multi-Agent Conversation

AutoGen is an open-source framework that allows developers to build LLM applications via multiple agents that can converse with each other to accomplish tasks. AutoGen agents are customizable, conversable, and can operate in various modes that employ combinations of LLMs, human inputs, and tools. Using AutoGen, developers can also flexibly define agent interaction behaviors. Both natural language and computer code can be used to program flexible conversation patterns for different applications. AutoGen serves as a generic infrastructure to build diverse applications of various complexities and LLM capacities. Empirical studies demonstrate the effectiveness of the framework in many example applications, with domains ranging from mathematics, coding, question answering, operations research, online decision-making, entertainment, etc.

==> figures/optiguide_compare_table.tex <==
\begin{table}[]
\caption{ChatGPT+ Code Interpreter vs. our autogen implementation of OptiGuide}
\label{tab:optiguide}
\begin{tabular}{c|p{7cm}|p{7cm}}
\toprule
\textbf{Action} & \textbf{ChatGPT+ Code Interpreter}          & \textbf{Autogen (ours)}      \\
\midrule
Setup & Customer open Web browser             & Setup OptiGuide service in 10 lines of code, and Customer open web browser    \\
\midrule
\faUser & \begin{tabular}[t]{p{6.5cm}}For the source code ``coffee.py",\\Can you tell me:\\What if we prohibit shipping from supplier 1 to roastery 2?\end{tabular}      & What if we prohibit shipping from supplier 1 to roastery 2? \\
\midrule
\faAndroid &   \begin{tabular}[t]{p{6.5cm}}
Because of proprietary package is used, we can not run the code. Download the new code, and run locally.
Copy + Paste the result to browser and query GPT again:\\ \\ Can you give me the explaination from the above execution results?\end{tabular}  & After adding the constraint to prohibit shipping from supplier 1 to roastery 2, the optimization problem was still solved successfully. The new objective value, which represents the minimum cost in this scenario, is 2760.0.  Compared to the original results without the constraint, where the optimal cost was 2470.0, the new solution is more expensive by 290 units. This shows that prohibiting shipping from supplier 1 to roastery 2 increases the total cost of the coffee distribution.\qed \\
\midrule
\faUser &  \begin{tabular}[t]{p{6.5cm}}Obtain the terminal results:\\Optimizer version 9.5.1 build v9.5.1rc2 (linux64)\\Thread count: 64 physical cores, 128 logical processors, using up to 32 threads\\{[}63 lines of output ignored{]}\\Best objective 2.760000000000e+03, best bound 2.760000000000e+03, gap 0.0000\%\\Wed Jul 26 09:49:59 2023\\Optimal cost: 2760.0\end{tabular}  &                              \\
\midrule
\faAndroid & After adding the constraint to prohibit shipping from supplier 1 to roastery 2, the optimization problem was still solved successfully. The new objective value, which represents the minimum cost in this scenario, is 2760.0.  Compared to the original results without the constraint, where the optimal cost was 2470.0, the new solution is more expensive by 290 units. This shows that prohibiting shipping from supplier 1 to roastery 2 increases the total cost of the coffee distribution.\qed  &   \\
\bottomrule
\end{tabular}
\end{table}









==> figures/optiguide_system.tex <==

% \begin{figure*}[h]
%     \centering
% 
% % Define the boxes
% \tikzstyle{user} = [ellipse, rounded corners, minimum width=3cm, minimum height=1cm,text centered, draw=black, fill=yellow!30]
% 
% \tikzstyle{tool} = [rectangle, dashed, minimum width=0.1cm, minimum height=0.1cm, text centered, draw=black, fill=green!10]
% \tikzstyle{agent} = [rectangle, rounded corners, minimum width=3cm, minimum height=1.2cm, text centered, draw=black, fill=green!30]
% 
% \tikzstyle{text_box} = [rectangle, minimum width=1mm, minimum height=1mm, text centered, draw=white]
% 
% 
% \tikzstyle{arrow} = [thick,->,>=latex]
% \tikzstyle{double_arrow} = [thick,<->,>=latex]
% 
% \begin{tikzpicture}[node distance=1cm]
% 
% % User
% \node (user) [user] {{\Large \faUser} User};
% 
% % OptiGuide agents
% \node (opti) [agent, minimum height=1.5cm, fill=blue!30, below=15mm of user] { Commander};
% % \node (tool) [tool, fill=green!20, below=-5mm of opti] {\small Tools};
% 
% % Big circle with arrow looping around the agents
% \draw[->, thick, dashed , gray!80, dash pattern=on 2pt off 2pt, line width=1.5pt ] ($(opti.west)$) arc (110:360:60mm and 20mm) arc (0:85:50mm and 20mm);
% \node (looping) [text_box, text=gray, text width=3 cm, below=1mm of opti, fill=white, xshift=60mm] {\small Repeat until answering the user's question or timeout};
% % \node (loop_text) [text_box, below=5mm of opti, xshift=10mm] 
% 
% \node (writer) [agent, fill=blue!30, below=15mm of opti, xshift=-35mm] {Writer};
% \node (safeguard) [agent, fill=blue!30, below=15mm of opti, xshift=35mm] {Safeguard};
% 
% 
% % optiguide frame
% % \node (opti_frame) [draw, rounded corners, dashed, gray!80, dash pattern=on 2pt off 2pt, line width=1.5pt, fit= (writer) (safeguard) (tool)   (opti)]  {};
% 
% % User - Optiguide
% \draw [arrow] ([xshift=-2mm] user.south) -- ([xshift=-2mm] opti.north) node[midway, left] {\small \circled{1} User question};
% \draw [arrow] ([xshift=2mm] opti.north) -- ([xshift=2mm] user.south) node[midway, right] {\small \circled{8} Final Answer};
% 
% % OptiGuide - Writer 
% \draw [arrow] ([yshift=3mm] opti.west) -- ([xshift=-3mm] writer.north) node[midway, sloped, above, fill=none] {\small \circled{2} Question, \shadeCircled{6} Log};
% \draw [arrow] ([xshift=3mm] writer.north) -- ([yshift=-3mm] opti.west) node[midway, sloped, below] {\small \shadeCircled{3} Code, \circled{7} Ans};
% 
% % OptiGuide - Safeguard
% \draw [arrow] ([yshift=3mm] opti.east) -- ([xshift=3mm] safeguard.north) node[midway, sloped, above] {\small \shadeCircled{4} Code};
% \draw [arrow] ([xshift=-3mm] safeguard.north) -- ([yshift=-3mm] opti.east) node[midway, sloped, below] {\small \shadeCircled{5} Clearance};
% 
% 
% 
% \end{tikzpicture}
% 
% 
%     \caption{Our re-implementation of \textit{OptiGuide} with autogen.agentchat. \todo{gb: use same format as rest of the paper.}}
%     \label{fig:optiguide}
% \end{figure*}


\begin{figure*}[h]
    \centering
    \includegraphics[width=0.8\linewidth]{figures/optiGuide_details.png}
    \caption{
Our re-implementation of \textit{OptiGuide} with \libName{} streamlining agents' interactions. The Commander receives user questions (e.g., What if we prohibit shipping from supplier 1 to roastery 2?) and coordinates with the Writer and Safeguard agents. The Writer crafts the code and interpretation, the Safeguard ensures safety (e.g., not leaking information, no malicious code), and the Commander executes the code. If issues arise, the process can repeat until resolved.
% \todo{[good-to-have] fix inconsistent font size}
    }
    \label{fig:optiguide}
\end{figure*}



==> figures/optiguide_table_long.tex <==
% What if the roasting cost is increased by 5\% because of the potential salary increase?

\section{Example outputs from applications}
\label{sec:example}

\begin{table*}[h!]
\caption{Application A1. Scenario 1: autonomous math solving. \libName on the first qualitative example. \libName solves the problem correctly.}
\label{tab:append_math_agentchat}
\small
\begin{tabular}{c|c|p{14cm}}
\toprule
 & \textbf{Action} & \textbf{\libName}     \\

\midrule
\faUser & Init chat & Completely simplify and rationalize the denominator: $$\frac{\sqrt{160}}{\sqrt{252}}\times\frac{\sqrt{245}}{\sqrt{108}}$$ \\
\midrule
\faAndroid  & & We can simplify and rationalize this denominator using Python's symbolic mathematics library `sympy`. Here is the Python code to resolve this:

\begin{lstlisting}
from sympy import sqrt, Rational

# Define the entire fraction as a rational number
fraction = (sqrt(160)/sqrt(252))*(sqrt(245)/sqrt(108))

# Simplify the fraction
simplified = fraction.simplify()

# Print the simplified fraction
print(simplified)
\end{lstlisting}

This code performs the requested simplification by constructing the fraction using the `Rational()` function from the `sympy` module, which automatically simplifies fractions when possible. The `sqrt()` function from the `sympy` module enables square root calculations. Finally, the `simplify()` function simplifies expressions when possible.
   \\

% \faUser & Code Reply &

\midrule
\faUser & Auto Code Reply & exitcode: 0 (execution succeeded)
Code output: 
5*sqrt(42)/27 \\
\midrule

\faAndroid  & & TERMINATE \\

\bottomrule
\end{tabular}
\end{table*}


\begin{table*}[h!]
\caption{Application A1. Scenario 1: autonomous math solving. LangChain ReAct on the first qualitative example. The code returns a decimal number.}
\label{tab:append_math_langchain}
\small
\begin{tabular}{c|c|p{14cm}}
\toprule
 & \textbf{Action} & \textbf{LangChain ReAct}     \\
 \midrule

\faUser & Input & Completely simplify and rationalize the denominator: $$\frac{\sqrt{160}}{\sqrt{252}}\times\frac{\sqrt{245}}{\sqrt{108}}$$ \\
\midrule
\faAndroid  & &  Entering new AgentExecutor chain...

To simplify this expression, I will first simplify each square root individually, then multiply the fractions as normal. The result should be a rational number.
Action: Python\_REPL
Action Input: 

\begin{lstlisting}
import math

# Calculate square roots
sqrt_160 = math.sqrt(160)
sqrt_252 = math.sqrt(252)
sqrt_245 = math.sqrt(245)
sqrt_108 = math.sqrt(108)

# Multiply fractions
numerator = sqrt_160 * sqrt_245
denominator = sqrt_252 * sqrt_108
result = numerator / denominator

print(result)
\end{lstlisting}

Observation: 1.200137166371826

Thought:I now know the final answer
Final Answer: The simplified and rationalized form of the expression is approximately 1.200137166371826.

Finished chain.
\\

\bottomrule
\end{tabular}
\end{table*}


\begin{table*}[h!]
\caption{Application A1. Scenario 1: autonomous math solving. ChatGPT+ Code Interpreter on the first qualitative example. The code returns a decimal number.}
\label{tab:append_math_wolfram}
\small
\begin{tabular}{c|c|p{14cm}}
\toprule
 & \textbf{Action} & \textbf{ChatGPT+ Code Interpreter}     \\
 \midrule

\faUser & Input & Completely simplify and rationalize the denominator: $$\frac{\sqrt{160}}{\sqrt{252}}\times\frac{\sqrt{245}}{\sqrt{108}}$$ \\
\midrule
\faAndroid  & & 

To simplify and rationalize the expression, we first simplify the radicals in the numerator and denominator by factoring out the largest perfect squares from the numbers under the square root. 

The perfect square factors of 160, 252, 245, and 108 are 16, 4, 1, and 36, respectively. Let's factorize and simplify: 

\[
\frac{\sqrt{160}}{\sqrt{252}}\times\frac{\sqrt{245}}{\sqrt{108}} = \frac{\sqrt{16 \times 10}}{\sqrt{4 \times 63}}\times\frac{\sqrt{245}}{\sqrt{36 \times 3}}
\]

We can simplify this further by applying the property \(\sqrt{ab} = \sqrt{a} \sqrt{b}\) and \(\frac{a}{b} \times \frac{c}{d} = \frac{a \times c}{b \times d}\).
\\

\faAndroid  & & 

Python
\begin{lstlisting}
import math

# factoring the square roots
sqrt_160 = math.sqrt(16) * math.sqrt(10)
sqrt_252 = math.sqrt(4) * math.sqrt(63)
sqrt_245 = math.sqrt(245)
sqrt_108 = math.sqrt(36) * math.sqrt(3)

# simplify the fraction
numerator = sqrt_160 * sqrt_245
denominator = sqrt_252 * sqrt_108
simplified_fraction = numerator / denominator

simplified_fraction

\end{lstlisting}

Result:
\begin{lstlisting}
1.200137166371826
\end{lstlisting} \\


\faAndroid  & & 

The completely simplified and rationalized form of the given expression is approximately \(1.200\). \\
\bottomrule
\end{tabular}
\end{table*}


\begin{table*}[h!]
\caption{Application A1. Scenario 1: autonomous math solving. ChatGPT+ Plugin (Wolfram Alpha) on the first qualitative example. Response from wolfram contains the correct answer but ChatGPT choosed the wrong answer.}
\label{tab:append_math_wolfram}
\small
\begin{tabular}{c|c|p{14cm}}
\toprule
 & \textbf{Action} & \textbf{ChatGPT+ Plugin}     \\
 \midrule

\faUser & Input & Completely simplify and rationalize the denominator: $$\frac{\sqrt{160}}{\sqrt{252}}\times\frac{\sqrt{245}}{\sqrt{108}}$$ \\
\midrule

\faAndroid  & & 

REQUEST TO WOLFRAM:

\begin{lstlisting}
{
  "input": "simplify (sqrt(160)/sqrt(252))*(sqrt(245)/sqrt(108))"
}
\end{lstlisting}

RESPONSE FROM WOLFRAM
\begin{lstlisting}
Query:
"simplify (sqrt(160)/sqrt(252))*(sqrt(245)/sqrt(108))"

Input interpretation:
simplify | sqrt(160)/sqrt(252)x sqrt(245)/sqrt(108)

Results:
(5 sqrt(42))/27

(5 sqrt(14/3))/9

Decimal approximation:
1.2001371663718259686974013770533327143898526494552493610576582218...

Wolfram|Alpha website result for "simplify (sqrt(160)/sqrt(252))*(sqrt(245)/sqrt(108))":
https://www.wolframalpha.com/input?i=simplify+%28sqrt%28160%29%2Fsqrt%28252%29%29%2A%28sqrt%28245%29%2Fsqrt%28108%29%29
\end{lstlisting}
\\


\faAndroid  & & 

The completely simplified and rationalized form of the given expression is:

$$\frac{5 \sqrt{14/3}}{9}$$

In decimal form, this is approximately 1.200137166371825968697401377053332714389852649...
\\

\bottomrule
\end{tabular}
\end{table*}




\begin{table*}[h!]
\caption{Application A1. Scenario 1: autonomous math solving. Auto-GPT on the first qualitative example. We abort since the code never prints the result and the system does not fix it after 2 turns. Auto-GPT is much more verbose than other frameworks. We shortened some of the unnecessary contents.}
\label{tab:append_math_wolfram}
\tiny
\begin{tabular}{c|c|p{14cm}}
\toprule
 & \textbf{Action} & \textbf{Auto-GPT}     \\
 
\midrule
  & System & 
Welcome back!  Would you like me to return to being MathSolverGPT?
  Asking user via keyboard...
Continue with the last settings?\newline
Name:  MathSolverGPT\newline
Role:  an intelligent math-solving AI that assists students, professionals,... \newline
Goals: ['Provide step-by-step solutions to math problems, ensuring clarity and understanding for the user... \newline
Continue (y/n): 
\\

\midrule
\faUser & Human input  & y
\\
\midrule

& System & MathSolverGPT  has been created with the following details:
Name:  MathSolverGPT\newline
Role:  an intelligent math-solving AI that assists students, professionals, and enthusiasts in solving a wide range of math problems, from basic arithmetic to advanced calculus and beyond.\newline
Goals: 
-  Provide step-by-step solutions to math problems, ensuring clarity and understanding for the user.
-  Offer explanations and insights into the underlying concepts and principles behind the solutions, fostering a deeper understanding of mathematics.
-  Handle a variety of math problem types, including algebra, geometry, trigonometry, calculus, and more. ...
\\
\midrule

\faAndroid  & & 
MATHSOLVERGPT THOUGHTS:  Without a specific task or question, it's difficult to determine exactly one command to use. The user hasn't provided any context or problem to solve. \newline
REASONING:  The user's request is too vague. They haven't specified what they want me to do or what problem they want me to solve.\newline
PLAN: 
-  Ask the user for more information or a specific task.\newline
CRITICISM:  I should have asked the user for more information or a specific task in the first place.\newline
SPEAK:  Could you please provide more information or specify a task?\newline

NEXT ACTION:  COMMAND =  ARGUMENTS = \{\}
\\
\midrule
& System &  Enter 'y' to authorise command, 'y -N' to run N continuous commands, 'n' to exit program, or enter feedback for MathSolverGPT...
  Asking user via keyboard...\\
\midrule

\faUser & Human input & 
Completely simplify and rationalize the denominator: $$\frac{\sqrt{160}}{\sqrt{252}}\times\frac{\sqrt{245}}{\sqrt{108}}$$
\\
\midrule

\faAndroid  & & 

MATHSOLVERGPT THOUGHTS:  To solve this problem, I need to simplify and rationalize the denominator of the given expression. This involves simplifying the square roots and then multiplying the fractions. I can use Python's math library to calculate the square roots and perform the multiplication. \newline
REASONING:  The problem involves simplifying square roots and multiplying fractions. Python's math library provides functions for these operations.\newline
PLAN: 
-  Write a Python script to calculate the square roots and multiply the fractions.
-  Execute the script to get the simplified expression.
CRITICISM:  I need to ensure that I correctly calculate the square roots and perform the multiplication. I should also make sure to rationalize the denominator, as the problem specifies.\newline
SPEAK:  Let's simplify and rationalize the denominator of the given expression.\newline

NEXT ACTION:  COMMAND = execute\_python\_code ARGUMENTS = 


\begin{lstlisting}[basicstyle=\tiny]
{'code': 'import math\n\n# Calculate the square roots\nsqrt_160 = math.sqrt(160)\nsqrt_252 = math.sqrt(252)\nsqrt_245 = math.sqrt(245)\nsqrt_108 = math.sqrt(108)\n\n# Multiply the fractions\nresult = (sqrt_160 / sqrt_252) * (sqrt_245 / sqrt_108)\n\n# Simplify the result\nsimplified_result = math.simplify(result)\n\nsimplified_result', 'name': 'simplify_expression'}
\end{lstlisting}
\\
\midrule

\faUser & Human input  & y
\\
\midrule

& System & 
-=-=-=-=-=-=-= COMMAND AUTHORISED BY USER -=-=-=-=-=-=-= \newline
Executing python file '/app/autogpt/workspa...

SYSTEM:  Command execute\_python\_code returned: Error: Traceback (most recent call last): File "...", line 13, in <module> simplified\_result = math.simplify(result) AttributeError: module 'math' has no attribute 'simplify'

\\

\midrule
\faAndroid & & 
MATHSOLVERGPT THOUGHTS:  The error message indicates that the 'math' module in Python does not have a 'simplify' function. I need to use the 'sympy' library instead, which provides a function for simplifying expressions.\newline
REASONING:  The 'math' module in Python does not provide a function for simplifying expressions. The 'sympy' library, on the other hand, does provide such a function.\newline
PLAN: 
-  Rewrite the Python script to use the 'sympy' library instead of the 'math' module.
-  Execute the script to get the simplified expression.
CRITICISM:  I should have known that the 'math' module does not provide a function for simplifying expressions. I should have used the 'sympy' library from the start.
SPEAK:  Let's try again using the 'sympy' library to simplify the expression.\newline

NEXT ACTION:  COMMAND = execute\_python\_code ARGUMENTS = 
\begin{lstlisting}[basicstyle=\tiny]
{'code': 'import sympy as sp\n\n# Calculate the square roots\nsqrt_160 = sp.sqrt(160)\nsqrt_252 = sp.sqrt(252)\nsqrt_245 = sp.sqrt(245)\nsqrt_108 = sp.sqrt(108)\n\n# Multiply the fractions\nresult = (sqrt_160 / sqrt_252) * (sqrt_245 / sqrt_108)\n\n# Simplify the result\nsimplified_result = sp.simplify(result)\n\nsimplified_result', 'name': 'simplify_expression'}
\end{lstlisting}
\\
\midrule

\faUser & Human input & y
\\
\midrule

& System  &
SYSTEM:  Command execute\_python\_code returned:
\\
\midrule

\faAndroid  & & 

MATHSOLVERGPT THOUGHTS:  The command execution didn't return any output, which is unusual. It seems there might be an issue with the execution of the Python code. I need to debug this.\newline
REASONING:  The Python code execution should have returned a result. The absence of a result suggests that there might be an issue with the code or its execution.\newline
PLAN: 
-  Review the Python code to identify any potential issues.
-  If necessary, modify the code and execute it again.
CRITICISM:  I should have ensured that the Python code was correct and would produce a result before executing it.
SPEAK:  It seems there was an issue with the execution of the Python code. Let's try again.\newline

NEXT ACTION:  COMMAND = execute\_python\_code ARGUMENTS = \begin{lstlisting}[basicstyle=\tiny]
{'code': 'import sympy as sp\n\n# Calculate the square roots\nsqrt_160 = sp.sqrt(160)\nsqrt_252 = sp.sqrt(252)\nsqrt_245 = sp.sqrt(245)\nsqrt_108 = sp.sqrt(108)\n\n# Multiply the fractions\nresult = (sqrt_160 / sqrt_252) * (sqrt_245 / sqrt_108)\n\n# Simplify the result\nsimplified_result = sp.simplify(result)\n\nsimplified_result', 'name': 'simplify_expression'}
\end{lstlisting}
\\
\midrule


 & System & 
SYSTEM:  Command execute\_python\_code returned:\\
\midrule
\faAndroid & &
MATHSOLVERGPT THOUGHTS:  The Python code execution still isn't returning any output. It's possible that the issue lies with the calculation of the square roots ...
\\
\midrule

\faUser  & Human input & 
control + C (Aborted)
\\
\bottomrule
\end{tabular}
\end{table*}


\begin{table*}[h!]
\caption{Application A2. ChatGPT+ Code Interpreter for OptiGuide. A sample question ``What if the roasting cost is increased by 5\% because of the potential salary increase?" is asked.}
\label{tab:optiguide_gpt_complex}
\tiny
\begin{tabular}{c|c|p{14cm}}
\toprule
 & \textbf{Action} & \textbf{ChatGPT+ Code Interpreter}     \\
\midrule
\faUser & Prompt Writer & \begin{tabular}[t]{p{13cm}}Customer open Web browser.\\For the source code ``coffee.py",\\Can you tell me:\\\textit{What if the roasting cost is increased by 5\% because of the potential salary increase?}
\end{tabular}     \\
\midrule
\faAndroid &   &   \begin{tabular}[t]{p{13cm}}
Sure! Let's first take a look at the contents of the "coffee.py" file to understand the code and how the roasting cost is calculated. This will allow us to determine the effect of a 5\% increase in the roasting cost.\\
...\textit{several lines omitted}\\
Would you like me to modify the code to reflect the 5\% increase in roasting costs and run the modified code to observe the impact? If the code requires any specific input or parameters, please let me know!
\end{tabular} \\
\midrule
\faUser & Prompt Writer & Yes \\
\midrule
\faAndroid & & \begin{tabular}[t]{p{13cm}}
Great! Before proceeding, I'll need to ensure that the Gurobi solver is not being used in this code, as my current environment does not have access to Gurobi. If the code does indeed use Gurobi, we can still analyze the effect of the change in roasting costs by understanding the structure of the code.\\
...\textit{several lines omitted}\\
Alternatively, if you have access to a Gurobi license, you can make the necessary changes in the code and run it on your local machine. I can guide you through the process of making the necessary modifications to the code.\\
Would you like me to proceed with the code analysis and explanation, or would you like guidance on making the changes yourself?
\end{tabular} \\
\midrule
\faUser & Prompt Writer & You can give me the full code, and I can run the code locally myself. \\
\midrule
\faAndroid & & 
\begin{tabular}[t]{p{13cm}}
Certainly! I'll modify the code to reflect a 5\% increase in both the light and dark roasting costs, and then provide the full code for you to run locally.\\
...\\
Download Modified Coffee.py\\
If you have any questions or need further assistance, please feel free to ask!
\end{tabular}
\\
\midrule
\faUser &  Prompt Safeguard &  \begin{tabular}[t]{p{13cm}} Hi GPT, can you safecheck the generated code for me? \\ \textit{Upload the generated code.} \end{tabular}  \\
\midrule
\faAndroid &   &  DANGER \\
\midrule
\faUser & Prompt Writer &  I have tried to run your code. However, the code triggered our safeguard, and it is not safe to run. Try again. Hint: don't change roasting\_cost\_light or roasting\_cost\_light  variables.  \\
\midrule
\faAndroid &   &   \begin{tabular}[t]{p{13cm}}
I apologize for the oversight. It appears I made direct changes to the variables that could have led to issues with the code. Let's take a different approach by analyzing the code to identify the appropriate place to apply the 5\% increase in roasting costs.\\
...\\
Download Modified Safe Coffee.py\\
...
\end{tabular} \\
\midrule
\faUser &  Prompt Safeguard &  \begin{tabular}[t]{p{13cm}} Hi GPT, can you safecheck the generated code for me one more time? \\ \textit{Upload the generated code.} \end{tabular}  \\
\midrule
\faAndroid &   & DANGER \\
\midrule
\faUser & Prompt Writer &  I have tried to run your code again. However, the code triggered our safeguard, and it is not safe to run. Try again. Hint: don't change roasting\_cost\_light or roasting\_cost\_light  variables.
  \\
\midrule
\faAndroid &   &   \begin{tabular}[t]{p{13cm}}
I apologize for the continued confusion. \\
...\\
Download Final Modified Safe Coffee.py\\
...
\end{tabular} \\
\midrule
\faUser &  Prompt Safeguard &  \begin{tabular}[t]{p{13cm}} Hi GPT, can you safecheck the generated code for me one more time? \\ \textit{Upload the generated code.} \end{tabular}  \\
\midrule
\faAndroid &   &   SAFE \\
\midrule
\faUser & Run Code & \begin{tabular}[t]{p{6.5cm}}Obtain the terminal results:\\Optimizer version 9.5.1 build v9.5.1rc2 (linux64)\\Thread count: 64 physical cores, 128 logical processors, using up to 32 threads\\{[}63 lines of output ignored{]}\\Optimal cost: 2526.5 \end{tabular}                              \\
\midrule
\faUser & Prompt Writer & Here is the execution result. [\textit{Copy + Paste the terminal output here.}] Can you extract the final answer to me? Remember to compare with the original cost of 2470. \\
\midrule
\faAndroid  & & \begin{tabular}[t]{p{6.5cm}}
Certainly! The execution result you've provided indicates the optimal cost for the modified scenario, where the roasting costs were increased by 5\%. Here's the comparison: \\
Original Cost: 2470 \\
Modified Cost (with 5\% increase in roasting costs): 2526.5\\
The increase in roasting costs has led to an increase in the overall cost by 56.5, reflecting the impact of the potential salary increase on the roasting cost. \\
If you need any further insights or assistance, please let me know!  \end{tabular}   \\
\bottomrule
\end{tabular}
\end{table*}




\begin{table*}[h!]
\caption{Application A2. \libName with OptiGuide. The same question ``What if the roasting cost is increased by 5\% because of the potential salary increase?" is asked.}
\label{tab:optiguide_complex}
\small
\begin{tabular}{c|c|p{14cm}}
\toprule
 & \textbf{Action} & \textbf{\libName}     \\
 % \midrule
 % & Setup & Setup OptiGuide. \\
\midrule
\faUser & Prompt & \textit{What if the roasting cost is increased by 5\% because of the potential salary increase?} \\
\midrule
\faAndroid  & & After increasing the roasting costs by 5\%, I've re-calculated the optimal coffee distribution solution for the supply chain. As a result, the new optimal total cost has become 2526.5, compared to the initial cost of 2470.0. This indicates that the increased roasting costs have caused the overall distribution cost to rise by 56.5 units.
   \\
\bottomrule
\end{tabular}
\end{table*}



==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> sec_iclr/_sec_intro.tex <==
\section{Introduction}

% agentic approach is powerful

% how to multi agent ?

% its promising and feasible, heres why...


Large language models (LLMs) are becoming a crucial building block in developing powerful {\em agents} that utilize LLMs for reasoning, tool usage, and adapting to new observations~\cite{yao2022react,xi2023rise,wang2023survey} in many real-world tasks.
% \jy{better put survey here? like 
% \cite{xi2023rise,wang2023survey}}.
% robot lawyers (DoNotPay),
% Advanced Data Analytics,
% Bing Chat,
% Bard etc.
% These applications, however, typically require that the developers build handcrafted pipelines %(e.g., via LangChain or Semantic Kernel)
% or create a single agent that can interleave reasoning, actions, and observations~\cite{yao2022react}.
% Either case requires management of 
% user input,
% prompts,
% multiple LLM inference calls and outputs,
% tool use and memory.
% % 
% To propose a third, even powerful approach,
Given the expanding tasks that could benefit from LLMs and the growing task complexity, 
% limitation of a typical single agent on navigating complex tasks%regarding diversity and adaptability
% \ahmed{is that about diversity and adaptability or the ability to solve more complex tasks; single LLM call is fast but not accurate. multi-agent is more deliberate} \qw{revised to ``navigating complex tasks"}, \cw{revised again}
% \ryen{This is a bit of a jump. Why can't single LLMs handle these expanding tasks with all their extensive capabilities?} \cw{and the limitation of a single agent in terms of diversity and adaptability,} \qw{Added.}
% and the intrinsic weaknesses of using a single agent~\cite{liang-arxiv2023,du2023improving,bubeck2023sparks}, 
an intuitive approach to scale up the power of agents is to use multiple agents that cooperate.
% \cw{: on the one hand, LLMs are known to be stochastic and require guardrails; on the other hand, they are effective at criticizing.} 
Prior work suggests that multiple agents can help encourage divergent thinking~\cite{liang-arxiv2023}, improve factuality and reasoning~\cite{du2023improving}, and provide guardrails~\cite{wu2023empirical}.
% \gb{One reason is that while models can hallucinate and go off the rails, they are also effective at criticizing, providing essential guardrails for generations—highlighting the fundamental role of a critic in preventing generation errors.}
In light of the intuition and early evidence of promise, it is intriguing to ask the following question: %Is this multi-agent approach generally feasible and useful, and 
{\em how} can we facilitate the development of LLM applications that could span a broad spectrum of domains and complexities based on the multi-agent approach?
% {\em Why} is this approach generally feasible, and {\em how} can we
% facilitate the development of more applications based on this approach?

% Despite the application diversity, the development of different applications often necessitates common functionalities, such as orchestrating multiple LLM agents, managing the interleaved LLM generation and tool execution, as well as integrating human inputs. Addressing these shared requirements can greatly facilitate the development of LLM applications broadly, and we have the insight that it can be achieved through a multi-agent conversation framework. 

Our insight is to use \emph{multi-agent conversations} to achieve it. 
There are at least three reasons confirming its general feasibility and utility thanks to recent advances in LLMs: First, because chat-optimized LLMs (e.g., GPT-4) show the ability to incorporate feedback,  
LLM-agents can cooperate through {\em conversations} with each other or human(s), e.g., a dialog where agents provide and seek reasoning, observations, critiques, and validation. Second, because a single LLM can exhibit a broad range of capabilities (especially when configured with the correct prompt and inference settings), conversations between differently-configured agents can help 
combine
these broad LLM capabilities in a modular and complementary manner. 
{Third, LLMs have demonstrated ability to solve complex tasks when broken into simpler subtasks. Multi-agent conversations can enable this partitioning and integration in an intuitive manner.}
% \db{In paragraph 2, I think we should call out some of the different patterns that seem important.  First, having different personas/experts/agents allows a combination of divergent thinking (as you refer to in the first paragraph).  That is one key pattern.  Second, the generator/critic pattern seems important.  Third, the notion of hierarchy (task partitioning and integration) seems important.  I'd name these precisely and call them out.  The point to make is that we don't know what patterns work best, these are three patterns that seem foundational and there may be others, but the Autogen tools should accommodate all of the important ones.
% }



% Prior work \qw{Prior multi-agent work?} has in fact shown to encourage divergent thinking~\cite{liang-arxiv2023} and improve factuality and reasoning~\cite{du2023improving}.
% We believe that these reasons can be leveraged to build multi-agent workflows and make them work in an effective way to scale up the power of LLMs and enable the next generation of their applications.


% --2--
% there are some conceptual and systems attempts
%  <list attempts>
%  they have issue, including
%  specialized for tasks that are hard to extend
%  or conceptual frameworks that have no implementation
% challenges when trying to faciliate dev of more apps on this approach:
% Agent design: figuring out a design of an agent that is both general/reusable but also suitable for a multi agent collaboration
% Agent communication paradigm: is how to create a simple, unified interface that can accommodate a variety of agents, various topologies, dynamic and static interactions, single- \& multi-turn dialogs, allow dev to program the control flow (in NL and PL)


% --3--
% we propose oss library autogen 
% autogen addressed these challenges
% 1. conversable agents
% 2. 

% \qw{The following paragraph is written based on the outline above.}

%In fact, several very recent\footnote{Note for reviewers: As of September 23rd, 2023 (ICRL submission deadline), none of these prior multi-agent approaches have been published at peer-reviewed venues and most appeared online after May 2023.} works have leveraged multi-agent approaches including CAMEL~\cite{li2023camel}, MetaGPT~\cite{hong2023metagpt}, BabyAGI~\cite{babyagi}, Multi-agent debate~\cite{du2023improving}, CHATDEV~\cite{qian2023communicative}, and AgentVerse~\cite{chen2023agentverse}. However, these works either proposed task-specific solutions which make them hard to extend or they proposed general conceptual frameworks without effective agent implementation (see Table~\ref{tab:relevant_work_compare}). 

% Despite the application diversity, the development of different applications often necessitates common functionalities, such as orchestrating multiple LLM calls, managing the interleaved LLM generation and tool execution, as well as integrating human inputs. Addressing these shared requirements can greatly facilitate the development of LLM applications broadly, and we have the insight that it can be achieved through a multi-agent conversation framework. 
% We desire a multi-agent conversation framework with both implementation support and flexibility to satisfy different application needs.
How can we leverage the above insights and support different applications with the common requirement of coordinating multiple agents, potentially backed by LLMs, humans, or tools exhibiting different capacities? %managing the interleaved LLM generation and tool execution, as well as integrating human inputs, 
We desire a multi-agent conversation framework with generic abstraction and effective implementation that has the flexibility to satisfy different application needs.
%support diverse applications in the future.
%\gb{``to support ... future'' is redundant with first clause; meaning of ``effective'' is missing}
%easy-to-extend. 
%In order to facilitate development of new applications based on multi-agent approaches, addressing these problems is crucial. 
Achieving this requires addressing two critical questions:
% This problem is inherently challenging.
% But there are several reasons that make this problem inherently challenging. 
% There are several challenges when trying to facilitate the development of more applications on this approach. 
% One significant challenge is related to agent design -- 
(1) How can we design individual agents that are capable, reusable, customizable, and effective in multi-agent collaboration? (2) How can we develop a straightforward, unified interface that can accommodate a wide range of agent conversation patterns? %These questions exist because
In practice, applications of varying complexities may need distinct sets of agents with specific capabilities, and may require different conversation patterns, such as single- or multi-turn dialogs, different human involvement modes, and static vs. dynamic conversation. Moreover, developers may prefer the flexibility to program agent interactions in natural language or code. Failing to adequately address these two questions would limit the framework's scope of applicability and generality.
% a variety of agents, diverse agent conversation patterns, 
%single- \& multi-turn dialogs, 
% flexible human involvement patterns, etc., needed by different applications while giving developers the flexibility to program the conversations
%control flow 
% between agents in natural language or code?
% \gb{q2 is long and convoluted. separate the essential and non essential using better sentence structure}
%Answering these questions is not trivial.
% \gb{please double check these two questions carefully}

% \gb{add para break here?}
While there is contemporaneous %\jy{contemporaneous?} 
exploration of multi-agent approaches,\footnote{As of September 23rd, 2023, most prior multi-agent LLM approaches have not been published at peer-reviewed venues and only appeared online after May 2023. Hence, per the ICLR reviewer guide they should be considered as contemporaneous work.
We refer to Appendix~\ref{sec:related_work} for a detailed discussion.}
% we take a generalized multi-agent conversational approach with broader applicability.
% our aim is to target a broader scope and applicability.%\gb{of generality $\rightarrow$ and generality}
%\gb{text needs to say what will happen if these questions are not answered}
% \gb{cut the last clause}
% \db{At the end of paragraph 3, you say "our aim is to arget a broader scope and achieve greater generality".  I would not make this claim.  I would say what specific technical approach you are taking that is differentiated and then show in the paper why it achieves the goals you said in this sentence.}
% \gb{remove para breask}
\comment{
\db{why will this paper win an award in 10 years?}
\gb{One way to do this would be to establish that is the correct way to think about multi agent systems} \cw{+1. LLM-powered multi-agent systems.}
Large Language Models (LLMs), like GPT-4, have demonstrated
exceptional capabilities for reasoning, creativity, and deduction in many new AI applications, ranging from robot lawyers~\cite{donotpay},
tools to assist with fundamental research~\cite{bran-arxiv2023},
and numerous highly-capable chatbots (e.g., Bing Chat, ChatGPT+, Copilot, Bard). 
Since single LLM calls lack ability to reflect, possess no working memory or scratch pad, and cannot act or perceive beyond the knowledge obtained from their training data~\cite{bubeck2023sparks}, augmenting language models with tools that facilitate perception and action (e.g., the plugin that enables ChatGPT+ to utilize fresh web pages from the internet~\cite{gptPlugin}) can significantly improve performance.

Despite the success of this LLM-with-tools paradigm~\cite{qin2023tool}, these approaches typically utilize a single LLM agent.\ahmed{Should we make an analogy to a single LLM call exhibiting system 1 behavior (fast, but can be error-prone) and multi-agent LLM-systems exhibiting system 2 behavior (deliberate, slow but more accurate and more capable)} \cw{Shall we start the paper from the next sentence?} Given the evolving range of real-world tasks that could benefit from LLMs and the intrinsic weaknesses of using a single agent~\cite{liang-arxiv2023,du2023improving,bubeck2023sparks}, a promising direction for future LLM applications is to use multiple agents that work together to solve complex tasks.
\db{This is not a new idea. What are you adding that is novel/unique}
\gb{Something along the lines of "our way is better way" could address this.} \cw{Previous work is specific or limited. Our work is a generalization of them, including our own prior work (2).}\gb{we provide evidence of importance of conversations}
For instance, additional agents could (1) encourage divergent thinking by allowing different roles ~\cite{liang-arxiv2023}, improve factuality and reasoning with LLMs through multi-agent debate~\cite{du2023improving}, etc; (2) allow effective tool usage and execution with potentially autonomous troubleshooting through inter-agent interactions~\cite{wu2023empirical}; (3) realize human agency to steer these agents, etc. \ahmed{the relation between multi-agent framework and human agency is not clear} 
In such multi-agent systems, inter-agent conversations will be crucial, using language (natural or code) as means to enable agent collaboration through potential multi-round, back-and-forth message exchanges. These conversations could  leverage the recent chat-based LLMs' capability to communicate and incorporate feedback from others at human level. 

% \note{Make the intro more concise? Especially the first and second paragraphs.}

 A unified framework that uses conversations between multiple agents can encapsulate the aforementioned insights in a general manner. 
%  Consider, for example, a developer building an application that uses LLMs to write code that solves a problem specified by a user (e.g., {\em``Plot a chart of META and TESLA stock price change YTD''}). The simplest starting point is to use a single LLM inference call to generate code. Since this code may be erroneous, the developer may use a separate tool to execute candidate code, and 
% subsequent LLM inference calls to debug the code based on execution results --- resulting in an iterative conversation between the inference and code execution. 
% Additionally, the developer may want to let users approve code execution, clarify their intent, and remember their preferences. Designing, implementing, and optimizing this workflow can be challenging. However, using well-designed agents and multi-agent conversations, the workflow could potentially be simplified into a series of discussions between the involved agents (Figure~\ref{fig:agent_capabilities}).
% To support the rapid development of next-gen LLM applications, an ideal framework would support the latest LLMs and augmentations, allow 
% (potentially automated) cooperation between LLMs, tools,
% and seamless and flexible human involvement to leverage their expertise and intelligence. 
}
%To foster progress with experimentation and development of multi-agent LLM-based applications, To this end, To this end, 
% To foster progress on this endeavor, 
% \gb{cut last clause} 
we develop \libName,
% \db{Need a concept name and project name.}
% \gb{This requires discussion} \cw{let's start by understanding why conversation programming is not good enough.}
a generalized multi-agent conversation framework (Figure~\ref{fig:landing}),
% \libName introduces 
based on the following new concepts.
% to answer the above  challenging questions:
% \db{The next few lines "to foster progress on this endeavor" should be rewritten, again, not to make bold general claims but to be specific about the design points you are including.}
\begin{enumerate}[leftmargin=*]
    \vspace{-2mm}
    \setlength\itemsep{-0.1em}
    \item[1] \textbf{Customizable and conversable agents.} \libName uses a generic design of agents that can leverage LLMs, human inputs, tools, or a combination of them. 
    %uses a design of agents that makes it feasible for them use to capabilities including LLMs, human input, tools, or a combination of these. 
    The result is that developers can easily and quickly create agents with different roles (e.g., agents to write code, execute code, wire in human feedback, validate outputs, etc.) by selecting and configuring a subset of built-in capabilities. The agent's backend can also be readily extended to allow more custom behaviors.  %(Section~\ref{sec:agent})
    % One key philosophy of \libName is to simplify and unify complex workflows as multi-agent conversations. To realize this, every \libName
    %\ryen{What's the difference between the libName and the AutogenAgent name?} \cw{Should be libName} 
    To make these agents suitable for multi-agent conversation, every
    agent is made {\em conversable}
    -- they can receive, react, and respond to messages. 
     When configured properly, an agent can hold multiple turns of conversations with other agents autonomously or solicit human inputs at certain rounds, enabling human agency and automation.
     The conversable agent design leverages the strong capability of the most advanced LLMs in taking feedback and making progress via chat
    and also allows combining capabilities of LLMs in a modular fashion.   (Section~\ref{sec:agent}) 
%\db{more precise}  \qw{Added one sentence.}
% When configured properly, an agent can hold multi-turns of conversation with other agents autonomously or solicit human inputs at certain rounds, enabling human agency and automation. 
    \item[2] \textbf{Conversation programming.} 
    %We have the insight that multi-agent conversations can be used to address the shared requirements of different applications efficiently and consider simplifying and unifying complex LLM applications workflows as a fundamental principle of \libName. 
    A fundamental insight of \libName is to simplify and unify complex LLM application workflows as multi-agent conversations.
    So \libName adopts a programming paradigm centered around these inter-agent conversations. We refer to this paradigm as \emph{conversation programming},  which streamlines the development of intricate %workflows 
    applications
    via two primary steps: (1) defining a set of conversable agents with specific capabilities
    and roles (as described above); (2) programming the interaction behavior between agents via conversation-centric \emph{computation} and \emph{control}. %To accomplish the latter, developers can use both natural language and code to build and experiment with a wide range of conversation patterns,
    % agent behavior,
    % the number of agents, and 
    % topology of agent interactions
    % (Section~\ref{sec:autogen_conv}). 
    Both steps can be achieved via a fusion of natural and programming languages to build applications with a wide range of conversation patterns and agent behaviors. \libName provides ready-to-use implementations and also allows easy extension and experimentation for both steps. 
    (Section~\ref{sec:autogen_conv})
% % \db{topological experimentation with gates?} 
% \gb{need to ensure this concept is clear and meaty}
    
\end{enumerate}
% We introduce \libName in Section~\ref{sec:framework}, review related work in Section~\ref{sec:related_work}, present applications in Section~\ref{sec:app}, and summarize the learnings and future work in Section~\ref{sec:summary}.

\libName also provides a collection of multi-agent applications created using conversable agents and conversation programming.
%, along with general guidelines. %These applications span a wide range of domains and complexities. 
These applications demonstrate how \libName can easily %support different conversation patterns to
support applications of various complexities and LLMs of various capabilities. 
Moreover, we perform %comprehensive evaluation including 
both evaluation on benchmarks and a pilot study of new applications. The results show that \libName can help achieve outstanding performance on many tasks, and enable innovative ways of using LLMs, while reducing the development % or operational \ahmed{how does it reduce operation effort?} \qw{it can save manual effort on code execution in some applications, e.g., 3x-5x human effort saving in OptiGuide compared with a system that cannot do integrated local code execution, e.g., ChatGPT + code interpreter} 
effort. (Section~\ref{sec:app} and Appendix~\ref{append:application})  
    
    % \db{why does this matter} \cw{empirical proof that the framework works.} \ahmed{+1 to why does this matter? still not clear. Maybe pivot on them being demonstrations of use cases with empirical results}


